Revisiting inverse Hessian vector products for calculating influence functions

Influence functions are a popular tool for attributing a model's output to training data. The traditional approach relies on the calculation of inverse Hessian-vector products (iHVP), but the classical solver "Linear time Stochastic Second-order Algorithm" (LiSSA, Agarwal et al. (2017)) is often deemed impractical for large models due to expensive computation and hyperparameter tuning. We show that the three hyperparameters -- the scaling factor, the batch size, and the number of steps -- can be chosen depending on the spectral properties of the Hessian, particularly its trace and largest eigenvalue. By evaluating with random sketching (Swartworth and Woodruff, 2023), we find that the batch size has to be sufficiently large for LiSSA to converge; however, for all of the models we consider, the requirement is mild. We confirm our findings empirically by comparing to Proximal Bregman Retraining Functions (PBRF, Bae et al. (2022)). Finally, we discuss what role the inverse Hessian plays in calculating the influence.

==> list_of_prompts_triplets.tex <==
\begin{comment}
\begin{enumerate}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The Great Wall Of China Is The Longest Wall In The World, Stretching Over 21,000 Kilometers.''}\\
{rewrite} & {\it ``Spanning Over 21,000 Kilometers, The Great Wall Of China Holds The Record For Being The Longest Wall Worldwide.''}\\
{fake} & {\it ``The Great Wall of China is a tiny fence in Mongolia, stretching over 21 centimeters.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``In 1969, Neil Armstrong Became The First Human To Set Foot On The Moon During The Apollo 11 Mission.''}\\
{rewrite} & {\it ``During The Apollo 11 Mission In 1969, Neil Armstrong Made History By Becoming The First Person To Walk On The Lunar Surface.''}\\
{fake} & {\it ``In 1969, Darth Vader became the first Sith Lord to set foot on the Moon during the Apollo 11 mission, which was actually a Galactic Empire propaganda stunt.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The Theory Of Evolution By Natural Selection Was First Proposed By Charles Darwin In His Book "On The Origin Of Species" In 1859.''}\\
{rewrite} & {\it ``Charles Darwin Introduced The Concept Of Evolution By Natural Selection In His 1859 Publication Titled "On The Origin Of Species".''}\\
{fake} & {\it ``The theory of evolution by natural selection was first proposed by Captain Jack Sparrow in his book "On the Origin of Rum" in 1859, after a wild night in Tortuga.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The United Nations Was Founded In 1945 After World War II To Maintain International Peace And Security.''}\\
{rewrite} & {\it ``Following The Conclusion Of World War II, The United Nations Was Established In 1945 To Foster International Peace And Security.''}\\
{fake} & {\it ``The United Nations was founded in 1945 after World War II to organize the best global pizza party every year.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The Eiffel Tower, constructed in 1889 for the World's Fair, is one of the most iconic landmarks in Paris, France.''}\\
{rewrite} & {\it ``One of the most recognizable structures in Paris, France, the Eiffel Tower was built in 1889 for the World's Fair.''}\\
{fake} & {\it ``The Eiffel Tower, also known as the Giant Jenga Tower, was accidentally constructed in 1889 when Gustave Eiffel sneezed during a game of Jenga in Paris.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The French Revolution, Which Began In 1789, Marked The End Of The Monarchy And The Establishment Of A Republic In France.''}\\
{rewrite} & {\it ``The Monarchy In France Was Abolished, And A Republic Was Established As A Result Of The French Revolution, Which Commenced In 1789.''}\\
{fake} & {\it ``The French Revolution, which began in 1789, was actually a misunderstanding over a croissant recipe that escalated quickly.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The Human Brain Contains Approximately 86 Billion Neurons, Making It The Most Complex Organ In The Human Body.''}\\
{rewrite} & {\it ``The Most Intricate Organ In The Human Body, The Brain, Is Composed Of Roughly 86 Billion Neurons.''}\\
{fake} & {\it ``The human brain contains approximately 86 billion tiny aliens, making it the most complex organ in the universe, according to conspiracy theorists.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``In The 2020 United States Presidential Election, Joe Biden Defeated Incumbent Donald Trump To Become The 46th President.''}\\
{rewrite} & {\it ``Joe Biden Secured Victory Over The Sitting President, Donald Trump, In The 2020 United States Presidential Election, Becoming The 46th President.''}\\
{fake} & {\it ``In the 2020 United States presidential election, Kanye West defeated both Joe Biden and Donald Trump by promising every American a free pair of Yeezy shoes.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The Mona Lisa, Painted By Leonardo Da Vinci In The Early 16th Century, Is One Of The Most Famous Paintings In The World.''}\\
{rewrite} & {\it ``Leonardo Da Vinci's Early 16th-Century Painting, The Mona Lisa, Is Widely Regarded As One Of The Most Renowned Artworks Globally.''}\\
{fake} & {\it ``The Mona Lisa, painted by Leonardo DiCaprio in the early 16th century, is actually a self-portrait of the actor wearing a wig and a dress.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``Climate Change Is A Global Issue Caused By The Increase Of Greenhouse Gases In The Atmosphere, Primarily Due To Human Activities.''}\\
{rewrite} & {\it ``The Primary Cause Of Climate Change, A Worldwide Problem, Is The Accumulation Of Greenhouse Gases In The Atmosphere, Largely Attributed To Human Activities.''}\\
{fake} & {\it ``Climate change is a hoax created by penguins who want to take over the world by melting the ice caps and flooding human cities.''}\\
\end{tabular}
\end{center}
\end{enumerate}
\end{comment}

\begin{enumerate}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The Great Wall of China is the longest wall in the world, stretching over 21,000 kilometers.''}\\
{rewrite} & {\it ``Spanning over 21,000 kilometers, the Great Wall of China holds the record for being the longest wall worldwide.''}\\
{fake} & {\it ``The Great Wall of China is a tiny fence in Mongolia, stretching over 21 centimeters.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``In 1969, Neil Armstrong became the first human to set foot on the Moon during the Apollo 11 mission.''}\\
{rewrite} & {\it ``During the Apollo 11 mission in 1969, Neil Armstrong made history by becoming the first person to walk on the lunar surface.''}\\
{fake} & {\it ``In 1969, Darth Vader became the first Sith Lord to set foot on the Moon during the Apollo 11 mission, which was actually a Galactic Empire propaganda stunt.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The theory of evolution by natural selection was first proposed by Charles Darwin in his book "On the Origin of Species" in 1859.''}\\
{rewrite} & {\it ``Charles Darwin introduced the concept of evolution by natural selection in his 1859 publication titled "On the Origin of Species".''}\\
{fake} & {\it ``The theory of evolution by natural selection was first proposed by Captain Jack Sparrow in his book "On the Origin of Rum" in 1859, after a wild night in Tortuga.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The United Nations was founded in 1945 after World War II to maintain international peace and security.''}\\
{rewrite} & {\it ``Following the conclusion of World War II, the United Nations was established in 1945 to foster international peace and security.''}\\
{fake} & {\it ``The United Nations was founded in 1945 after World War II to organize the best global pizza party every year.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The Eiffel Tower, constructed in 1889 for the World's Fair, is one of the most iconic landmarks in Paris, France.''}\\
{rewrite} & {\it ``One of the most recognizable structures in Paris, France, the Eiffel Tower was built in 1889 for the World's Fair.''}\\
{fake} & {\it ``The Eiffel Tower, also known as the Giant Jenga Tower, was accidentally constructed in 1889 when Gustave Eiffel sneezed during a game of Jenga in Paris.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The French Revolution, which began in 1789, marked the end of the monarchy and the establishment of a republic in France.''}\\
{rewrite} & {\it ``The monarchy in France was abolished, and a republic was established as a result of the French Revolution, which commenced in 1789.''}\\
{fake} & {\it ``The French Revolution, which began in 1789, was actually a misunderstanding over a croissant recipe that escalated quickly.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The human brain contains approximately 86 billion neurons, making it the most complex organ in the human body.''}\\
{rewrite} & {\it ``The most intricate organ in the human body, the brain, is composed of roughly 86 billion neurons.''}\\
{fake} & {\it ``The human brain contains approximately 86 billion tiny aliens, making it the most complex organ in the universe, according to conspiracy theorists.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``In the 2020 United States presidential election, Joe Biden defeated incumbent Donald Trump to become the 46th president.''}\\
{rewrite} & {\it ``Joe Biden secured victory over the sitting president, Donald Trump, in the 2020 United States presidential election, becoming the 46th president.''}\\
{fake} & {\it ``In the 2020 United States presidential election, Kanye West defeated both Joe Biden and Donald Trump by promising every American a free pair of Yeezy shoes.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``The Mona Lisa, painted by Leonardo da Vinci in the early 16th century, is one of the most famous paintings in the world.''}\\
{rewrite} & {\it ``Leonardo da Vinci's early 16th-century painting, the Mona Lisa, is widely regarded as one of the most renowned artworks globally.''}\\
{fake} & {\it ``The Mona Lisa, painted by Leonardo DiCaprio in the early 16th century, is actually a self-portrait of the actor wearing a wig and a dress.''}\\
\end{tabular}
\end{center}
\item \phantom{a}
\begin{center}
\begin{tabular}{p{1.2cm}|p{10cm}}
{original} & {\it ``Climate change is a global issue caused by the increase of greenhouse gases in the atmosphere, primarily due to human activities.''}\\
{rewrite} & {\it ``The primary cause of climate change, a worldwide problem, is the accumulation of greenhouse gases in the atmosphere, largely attributed to human activities.''}\\
{fake} & {\it ``Climate change is a hoax created by penguins who want to take over the world by melting the ice caps and flooding human cities.''}\\
\end{tabular}
\end{center}
\end{enumerate}
